Gaussian Process Classification for Variable Fidelity Data

In this paper we address a classification problem where two sources of labels with different levels of fidelity are available. Our approach is to combine data from both sources by applying a co-kriging schema on latent functions, which allows the model to account item-dependent labeling discrepancy. We provide an extension of Laplace inference for Gaussian process classification, that takes into account multi-fidelity data. We evaluate the proposed method on real and synthetic datasets and show that it is more resistant to different levels of discrepancy between sources than other approaches for data fusion. Our method can provide accuracy/cost trade-off for a number of practical tasks such as crowd-sourced data annotation and feasibility regions construction in engineering design.

==> sections/3_4_theory.tex <==

% \section{Theory}
% \label{sec:theory}
% The theoretical section starts with a formal problem statement followed by a solution that extends Laplace Approximation for the multi-fidelity case.
% \input{sections/3_problem_statement}
% \input{sections/4_solution}

==> sections/3_m_and_ms.tex <==
% \section{Materials and methods}
% \label{sec:m_and_ms}

% In this section, we provide an overview of the technique called Laplace Approximation, that forms the basis of our multi-fidelity classification model based on GPs. Next, we introduce datasets and define evaluation metrics we used in the experiments.

% \subsection{Laplace Approximation}
% Prediction based on GPs requires two steps \cite{Rasmussen2006gaussianprocesses}: 1) obtaining a latent predictive distribution for the test point via marginalizing the posterior distribution over all possible latent values at train points, and 2) marginalizing it over all possible latent values at the test point in order to produce a probabilistic prediction. 

% Unlike regression problem, where marginalizations are straightforward because all underlying components are Gaussian, prediction of classes is analytically intractable due to non-Gaussian likelihoods.

% The idea of Laplace's method is to handle intractability at step 1 by applying a second order Taylor expansion of posterior's logarithm around its maximum. Thus we obtain a Gaussian approximation of the posterior distribution, which in turn makes approximate predictive distribution also Gaussian. Next, intractability of step 2 can be resolved by replacing marginalization with maximum a posteriori predictions \cite{bishop1995neural} or approximated with numerical techniques \cite{mackay1992evidence, williams1998bayesian}.

% Further, in this paper, we derive Laplace Approximation for multi-fidelity case based on that for single-fidelity, provided in section 3.4 in the book \cite{Rasmussen2006gaussianprocesses}. 


% \subsection{Evaluation metrics}
% In order to compare performance of various methods we use areas under receiver operating characteristic curves \cite{hanley1982meaning} (\ROCAUC{}) metric. 

% Further, to aggregate performance across many tests and datasets, we average \ROCAUC{} over them. We also  supplement results with figures of \emph{\ROCAUC{} profiles}, which show the share of tests where the corresponding methods had greater \ROCAUC{} than the threshold pointed on the abscissa axis. The rule of thumb for assessing such profiles is the higher the curve, the better the corresponding method.

% \subsection{Datasets}

% We evaluated our model on three groups of datasets: 
% \begin{enumerate}
%     \item Artificial datasets\footnote{We published them in this repository  \texttt{https://github.com/user525/mfgpc}}: we constructed datasets by virtue of the model \eqref{eq:model} and \eqref{eq:cokriging_dependency}. Latent functions $f_L$ and $\delta$ were generated as instances of Gaussian processes, linear coefficients $\rho$ were adjusted to the desired  discrepancy (noise level) between low- and high- fidelities. We used input dimensions 2, 5, 10, and 20. For each of them, we generated 10 datasets.
%     \item Datasets from Penn Machine Learning Benchmarks repository \citep{Olson2017PMLB}: we selected several representative benchmarks with different types of features, namely \texttt{diabetes} (\diabetes{}), \texttt{german} (\german{}), \texttt{waveform}-40 (\waveform{}), \texttt{satimage} (\satimage{}), \texttt{splice} (\splice{}), \texttt{spambase} (\spambase{}), \texttt{hypothyroid} (\hypothyroid{}), and \texttt{mushroom} (\mushroom{}). Since some datasets had multiple classes, we also selected one target representative class to test its classification against others: class 0 for \texttt{waveform-40} and \texttt{splice}, class 1 for \texttt{satimage} and class 2 for \texttt{diabetes}. Low-fidelity labels were generated by flipping original labels with the specified probability (noise level).
%     \item Real datasets: we used \texttt{music\_genre} (\musicgenre{}) and \texttt{sentiment\_polarity} (\sentimentpolarity{}) from \cite{rodrigues2014gaussian}, which had been annotated with crowd-sourcing. Each object in those datasets was labeled by multiple annotators, therefore we considered major voting statistic over object labels as high-fidelity and a single random annotation as low-fidelity. Such an approach to model fidelity is reasonable in the context to crowd-sourced annotations where each on them costs some amount of resources (e.g. money or time). For example, some objects are easy to classify with machine learning algorithms, thus one vote would be enough to annotate them, whereas for complex objects many votes are necessary for obtaining good confidence in labels. Finally, since \texttt{music\_genre} dataset had multiple classes, we tested each of them with the one-vs-all scheme as separate datasets. %\todo{\texttt{faces} dataset with NN features preprocessing?}
% \end{enumerate}
